Structural Subtyping as Parametric Polymorphism

Structural subtyping and parametric polymorphism provide similar flexibility and reusability to programmers. For example, both features enable the programmer to provide a wider record as an argument to a function that expects a narrower one. However, the means by which they do so differs substantially, and the precise details of the relationship between them exists, at best, as folklore in literature. In this paper, we systematically study the relative expressive power of structural subtyping and parametric polymorphism. We focus our investigation on establishing the extent to which parametric polymorphism, in the form of row and presence polymorphism, can encode structural subtyping for variant and record types. We base our study on various Church-style $\lambda$-calculi extended with records and variants, different forms of structural subtyping, and row and presence polymorphism. We characterise expressiveness by exhibiting compositional translations between calculi. For each translation we prove a type preservation and operational correspondence result. We also prove a number of non-existence results. By imposing restrictions on both source and target types, we reveal further subtleties in the expressiveness landscape, the restrictions enabling otherwise impossible translations to be defined. More specifically, we prove that full subtyping cannot be encoded via polymorphism, but we show that several restricted forms of subtyping can be encoded via particular forms of polymorphism.

==> Makefile <==
LATEXMK := $(shell command -v latexmk 2> /dev/null)

TEXC=pdflatex
CFLAGS=-interaction=nonstopmode -halt-on-error -file-line-error
BIBC=bibtex
PAPER=rowsub
BIBLIO=$(PAPER)

# Sam wants to use latexmk -- I don't. You can opt out of using
# latexmk by adding your username to the array OPT_OUT below.
BUILD_METHOD=$(PAPER).pdf
OPT_OUT := dhil

all:
  ifndef LATEXMK
    BUILD_METHOD=$(PAPER).pdf
  else
    ifneq ($(filter $(USER),$(OPT_OUT)),)
      BUILD_METHOD=$(PAPER).pdf
    else
      BUILD_METHOD=$(PAPER).pdf-via-latexmk
    endif
  endif
all: $(BUILD_METHOD)

extended: $(BUILD_METHOD)-extended
arxiv: $(BUILD_METHOD)-arxiv
camera-ready: all


crop: $(PAPER).pdf
	pdftk $(PAPER).pdf cat 1-29 output submission.pdf

$(PAPER).aux: $(PAPER).tex
	$(TEXC) $(CFLAGS) $(PAPER)

$(BIBLIO).bbl: $(PAPER).aux $(BIBLIO).bib
	$(BIBC) $(PAPER)

$(PAPER).pdf-arxiv: CFLAGS:=$(CFLAGS) "\def\ARXIV{}\input{$(PAPER)}"
$(PAPER).pdf-arxiv: all

$(PAPER).pdf-extended: CFLAGS:=$(CFLAGS) "\def\EXTENDED{}\input{$(PAPER)}"
$(PAPER).pdf-extended: all

$(PAPER).pdf: $(PAPER).aux $(BIBLIO).bbl
	$(TEXC) $(CFLAGS) $(PAPER)
	$(TEXC) $(CFLAGS) $(PAPER)

$(PAPER).pdf-via-latexmk: $(PAPER).tex
	latexmk -pdf $(CFLAGS) $(PAPER)

$(PAPER).pdf-via-latexmk-extended: $(PAPER).tex
	latexmk -pdf -pdflatex='pdflatex %O $(CFLAGS) -synctex=1 "\def\EXTENDED{}\input{%S}"' $(PAPER)

$(PAPER).pdf-via-latexmk-arxiv: $(PAPER).tex
	latexmk -pdf -pdflatex='pdflatex %O $(CFLAGS) -synctex=1 "\def\ARXIV{}\input{%S}"' $(PAPER)

clean:
	rm -f *.log *.aux *.toc *.out
	rm -f *.bbl *.blg *.fls *.xml
	rm -f *.fdb_latexmk *.vtc *.cut
	rm -f $(PAPER).pdf camera-ready.pdf submission.pdf
	rm -f *.o *.cmx *.cmo

